GC3: An Optimizing Compiler for GPU Collective Communication

Machine learning models made up of millions or billions of parameters are trained and served on large multi-GPU systems. As models grow in size and execute on more GPUs, the collective communications used in these applications become a bottleneck. Custom collective algorithms optimized for both particular network topologies and application specific communication patterns can alleviate this bottleneck and help these applications scale. However, correctly and efficiently implementing custom algorithms is challenging. This paper introduces GC3, a system for programmable GPU communication. GC3 provides a domain specific language for writing collective communication algorithms and an optimizing compiler for lowering them to an executable form, which can be executed efficiently and flexibly in an interpreter based runtime. We used GC3 to write novel collective algorithms for AllReduce and AllToAll that are up to $1.9\times$ and $1.3\times$ faster than hand-optimized implementations, respectively.

==> text/allreduce_program.tex <==
\begin{lstlisting}
# R = number of ranks
def ring_allreduce(R, ch):
  for i in range(R):
    c = chunk(i, 'out', i)

    # Compute fully reduced chunk
    for r in range(1, R):
      r = chunk((i+r)%R, 'out', i)
      c = r.reduce(c, ch=i%ch)

    # Broadcast fully reduced chunk
    for r in range(0, R-1):
      c = c.copy((i+r)%R, 'out', i, ch=i%ch)
\end{lstlisting}


==> text/alltoallhier_program.tex <==
\begin{lstlisting}
  # N: number of nodes
  # G: number of GPUs per node
  def alltoall_hierarchical(N, G):
  # input(m, i, n, j) -> gather(m, gr, gri) -> scatter(n, sr, sri) -> output(n, j, m, i)
  for m in range(N):
      for n in range(N):
          gr = gather_rank(m, n)
          gri = gather_index(m, n)
          sr = scatter_rank(m, n)
          sri = scatter_index(m, n)
          for i in range(G):
              for j in range(G):
                  c = chunk(m*G+i, 'input', n*G+j)
                  if n == m:
                      c.assign(n*G+j, 'output', m*G+i)
                  else:
                      c.assign(m*G+gr, 'gather', gri + i*G+j)

          if n == gr:
              # do a coalesced IB send 
              c = chunk(m*G+gr, 'gather', gri, G*G)
              c.assign(n*G+sr, 'scatter', sri)

              # local scatter
              for i in range(G):
                  for j in range(G):
                      c = chunk(n*G+sr, 'scatter', sri + i*G+j)
                      c.assign(n*G+j, 'output', m*G+i)
\end{lstlisting}

==> text/alltonext_program.tex <==
\begin{lstlisting}
def alltonext(N, G)
	for n in range(N): # N nodes
		for g in range(G): # G GPus per node
			if g != G-1: # direct intra-node send
				c = chunk((n, g), 'in', 0, sz=G)
				c.copy((n, g+1), 'out', 0)
				continue
			# last rank does not send anything
			if n == N-1:
				continue
			# use G IB links by routing through scratch buffers
			for i in range(G): `\label{line:alltonext_node_start}` 
				c = chunk('in', rank=(n,g), index=i)
				if i == 0:
					c = c.copy(rank=(n, 0), 'sc', 0)
					c.copy((n+1, 0), 'out', 0)
				elif i == G-1:
					c = c.copy((n+1, i), 'sc', 0)
					c.copy((n+1, 0), 'out', i)
				else:
					c = c.copy((n, i), 'sc', 0)
					c = c.copy((n+1), 'sc', 0)
					c.copy((n+1, 0), 'out', i) `\label{line:alltonext_node_stop}` 
\end{lstlisting}

==> text/extensions.tex <==
\subsection{\SCCLang Scheduling Extensions}
\label{sec:extensions}
\label{sec:manual-tb}

In this section we describe two extensions to \SCCLang{}, both of which give the user control over how instructions
are placed into thread blocks. 

\paragraph*{Manual Thread Block Assignment}
In many situations, a program's performance can be improved by manually scheduling it onto thread blocks.
This is accomplished with two additional optional parameters that can be given to the \lstinline{copy} and \lstinline{reduce}
operations in~\autoref{tbl:scclang}:

\begin{lstlisting}[language=Python, numbers=none, escapeinside={(*}{*)}]
    c.copy(rank, buf, idx, (*\bfseries sendtb*), (*\bfseries recvtb*))
    c1.reduce(c2, (*\bfseries sendtb*), (*\bfseries recvtb*))
\end{lstlisting}
The values given here directly replace the thread blocks indices that automatic assignment would infer. If these
arguments are used in any operation, then they must currently be used in every operation, since \SCCLang{} currently
doesn't support doing partial automatic thread block assignment.

\paragraph*{Channel Directives}
As an alternative to full manual thread block assignment, we allow users to specify the channel the operation must be performed on. 
Since no two thread blocks on the same GPU with the same send or receive peer can use the same channel, this allows forcing operations into different thread blocks. These channel directives are respected by the automatic thread block assignment when it considers candidate thread blocks. The channel are again specified with additional optional parameters:

\begin{lstlisting}[language=Python, numbers=none,   escapeinside={(*}{*)}]
    c.copy(rank, buf, idx, (*\bfseries ch*))
    c1.reduce(c2, (*\bfseries ch*))
\end{lstlisting}
We have used channel directives to ensure parallel sends over Infiniband while automatic thread block assignment was
sufficient for the rest of the program.


==> text/hierallreduce_program.tex <==
\newcommand{\indentrule}{\color{gray}\rlap{\smash{\hspace{3pt}\rule[-.35em]{1pt}{1.45em}}}}

\begin{lstlisting}
	# N: number of nodes
	# G: number of GPUs per node
	def HierarchicalAllReduce(N, G):
	# intra-node ReduceScatter
	for n in range(N):
		local_ranks = [i+n*G for i in range(G)]
		ReduceScatter(local_ranks, 0, N, 0)

	# inter-node ReduceScatter + AllGather
	for g in range(G):
		cross_ranks = [i*G+g for i in range(N)]
		ReduceScatter(cross_ranks, g*N, 1, 0)
		AllGather(cross_ranks, g*N, 1, 1)

	# intra-node AllGather
	for n in range(N):
		local_ranks = [i+n*G for i in range(G)]
		AllGather(local_ranks, 0, N, 2)


\end{lstlisting}


==> text/redscatallgat_program.tex <==
%\newcommand{\indentrule}{\color{gray}\rlap{\smash{\hspace{3pt}\rule[-.35em]{1pt}{1.45em}}}}

\begin{lstlisting}
# ranks = list of ranks involved 
# offset = offset into the input buffer
# count = num. of chunks sent at each step
# channel = channel assignment for the collective
def ReduceScatter(ranks, offset, count, channel):
	for r in range(0, len(ranks)):
		index = offset + r * count
		rank = ranks[(r+1)% len(ranks)]
		c = chunk(ranks, 'in', index, count)
		for step in range(1, len(ranks)):
			next = ranks[(step+r+1) % len(ranks)]
			dst_c = chunk(next, 'in', index, count)
			c = dst_c.reduce(c, channel)

def AllGather(ranks, offset, count, channel):
	for r in range(0, len(ranks)):
		index = offset + r * count
		c = chunk(ranks[r], 'in', index, count)
		for step in range(1, len(ranks)):
			next = ranks[(step+r)  % len(ranks)]
			c = c.copy(next, 'in', index, count, channel)


\end{lstlisting}

